Judge Anything: MLLM as a Judge Across Any Modality

Evaluating generative foundation models on open-ended multimodal understanding (MMU) and generation (MMG) tasks across diverse modalities (e.g., images, audio, video) poses significant challenges due to the complexity of cross-modal interactions. To this end, the idea of utilizing Multimodal LLMs (MLLMs) as automated judges has emerged, with encouraging results in assessing vision-language understanding tasks. Moving further, this paper extends MLLM-as-a-Judge across modalities to a unified manner by introducing two benchmarks, TaskAnything and JudgeAnything, to respectively evaluate the overall performance and judging capabilities of MLLMs across any-to-any modality tasks. Specifically, TaskAnything evaluates the MMU and MMG capabilities across 15 any-to-any modality categories, employing 1,500 queries curated from well-established benchmarks. Furthermore, JudgeAnything evaluates the judging capabilities of 5 advanced (e.g., GPT-4o and Gemini-2.0-Flash) from the perspectives of Pair Comparison and Score Evaluation, providing a standardized testbed that incorporates human judgments and detailed rubrics. Our extensive experiments reveal that while these MLLMs show promise in assessing MMU (i.e., achieving an average of 66.55% in Pair Comparison setting and 42.79% in Score Evaluation setting), they encounter significant challenges with MMG tasks (i.e., averaging only 53.37% in Pair Comparison setting and 30.05% in Score Evaluation setting), exposing cross-modality biases and hallucination issues. To address this, we present OmniArena, an automated platform for evaluating omni-models and multimodal reward models. Our work highlights the need for fairer evaluation protocols and stronger alignment with human preferences. The source code and dataset are publicly available at: https://urrealhero.github.io/judgeanythingweb/.

==> Section/2-related.tex <==
\section{Related Work}
% \header{LLM as a Judge}  
% With the introduction of MTBench \cite{LLM-as-a-judge}, LLMs have been explored as evaluation tools. Approaches such as GPTScore \cite{GPTScore}, HD-Eval \cite{HD-Eval}, and CLAIR \cite{CLAIR} have enhanced evaluation quality through prompt engineering, while MLLM-as-a-Judge \cite{mllm-as-a-judge} has extended these capabilities to image-based tasks. VBench \cite{Vbench} further leveraged MLLMs to evaluate video generation quality, and Llava-Critic \cite{LlavaCritic} emerged as one of the pioneering models employing MLLMs for evaluation.  
% As generative models continue to advance, there is an increasing demand to reduce reliance on human annotation in evaluation. Concurrently, AlignAnything \cite{AlignAnything} has explored the evaluation of \textit{any-to-any} generative tasks, further demonstrating the potential of AI-driven evaluation methodologies.

% \header{Any to Any Generation}
% The recent advancements in Transformer-based models \cite{transformer} and Diffusion models \cite{DDPM} have significantly impacted both natural language processing and computer vision, demonstrating their versatility across a variety of tasks. As the field shifts toward the development of generalist AI capable of handling multi-modal tasks, research has increasingly focused on transfer learning \cite{meta-transformer} and alignment learning \cite{nextgpt} to build robust Any-to-Any models. In this context, the use of auto-encoders has become widespread, with architectures like VAE \cite{vae} and VQ-VAE \cite{vqvae} playing pivotal roles in representation learning.
% As for encoder architectures, several models have emerged with innovative approaches to modality integration. Next-GPT, ModaVerse \cite{ModaVerse}, and Unified-IO2 \cite{unifiedIO2} adopt multi-projector frameworks to separately process and align different modalities within a shared latent space. On the other hand, models such as ImageBind-LLM \cite{imagebind} and PandaGPT \cite{pandagpt} utilize single-projector systems to encode all modalities simultaneously into a unified latent representation.
% In terms of generation, Next-GPT and the CoDi-series \cite{Codi} leverage diffusion models as generative models to produce high-quality content across various modalities. Alternatively, Teal \cite{Teal} and Mini-Omni2 \cite{Ocean-Omni} rely on autoregressive methods for modality-specific content generation, highlighting the flexibility of generative strategies in multi-modal AI systems.
% These advancements illustrate the diversity in approaches for encoding, alignment, and generation in multi-modal learning systems. As the research continues to evolve, hybrid models combining both diffusion and autoregressive techniques, as well as the exploration of more efficient encoding strategies, hold great promise for building more generalized Any-to-Any models.

\header{Multimodal Understanding (MMU).}
Multimodal Understanding (MMU) involves integrating and processing information from multiple modalities—such as text \citep{li2023cmmlu,li2023cmmlu}, images \citep{yue2024mmmu,zhang2024cmmmu}, video \citep{zhao2025mmvu,hu2025video}, audio \citep{sakshi2024mmau}—achieve significant development since the advent of MLLMs. Through late fusion of modality features with pretrained LLMs and modality instruction tuning \citep{liu2023visual}, MLLMs gain incredibly advanced understanding capabilities in images \citep{zhu2023minigpt,li2023blip}, videos \citep{lin2023video,zhang2023video}, audio \citep{chu2023qwen, chu2024qwen2}, and even interleaved content \citep{chen2025interleaved}.

Recent benchmarks like MMMU \citep{yue2024mmmu} and Video-MMMU \citep{hu2025video} have been developed to rigorously evaluate understanding and reasoning in \emph{specific modality} of MLLMs. \textit{Any-to-Any} benchmarks also emerge to provide comprehensive assessment for current well-rounded models capable of understanding in many modalities \citep{chen2024omnixr, li2024omnibench,ni2024mixeval,hong2025worldsense}. However, these benchmarks evaluate MMG mainly through Multiple-Choice QA, undermining the reliable assessment of real-world open-ended queries \citep{realworldqa2024}.

\header{Multimodal Generation (MMG).}
Multimodal Generation (MMG) involves generating content in one modality based on input from another or mixture \citep{ni2024mixeval,chen2025interleaved}, such as text-to-image \citep{ghosh2023geneval,T2IComp}, image-to-video \citep{V2VBench,fan2023aigcbench} and other modality transformations \citep{seung2023musiccaps,kang2024video2music,zhuo2023video}. Early approaches primarily focused on building specific framework for each task \citep{openai_dalle3,yang2024cogvideox}, which were later unified by Auto-Regressive (AR) models such as Emu-3 \citep{wang2024emu3}, and Unified-IO \citep{lu2022unified,unifiedIO2} which enabling understand and generate various modalities within a single backbone.

However, the open-ended nature of MMG tasks makes evaluation challenging, as traditional ground-truth-based metrics fail to capture the diversity and quality of generated content \citep{ni2024mixeval}. Human-oriented evaluations, such as those on crowdsourcing platforms like GenAI-Arena \citep{jiang2025genai} and other benchmarks \citep{liang2024rich,huang2024vbench}, have become a common approach to assess MMG tasks. Despite their utility, these platforms often suffer from issues like insufficient votes, leading to instability in rankings \citep{mllm-as-a-judge}. Our work advances the uniform incorporation of MLLM-as-a-Judge across various modalities by implementing \method reasoning to achieve more unbiased, reliable, and reproducible evaluations of MMG tasks.

\header{Multimodal LLM-as-a-Judge.}
Originated from Natural Language Generation (NLG) domain, LLM-as-a-Judge \citep{LLM-as-a-judge} have extended to multimodal domains serving as evaluation metrics in general QA \citep{mllm-as-a-judge,xiong2024llava,lee2024prometheus,tan2024judgebench}, image generation \citep{chen2024mj,lin2024evaluating}, video generation \citep{luo2024videoautoarena}, 3D synthesis \citep{wu2024gpt}, SWE tasks \citep{zhuge2024agent}, and interleaved generation \citep{chen2025interleaved,zhou2024gate}. Another line leverage pretrained MLLMs serving as reward models \citep{Yasunaga2025MultimodalRH,li2024vlrewardbench,yu2024rlaif,zhang2025mm,wang2024mllm} in aligning other MLLMs for advanced performance. MLLM-as-a-Judge \citep{mllm-as-a-judge} takes the first step in systematically quantifying MLLMs' performance as judges and assessing potential problems such as bias and hallucinations in Vision-Language Understanding tasks. Our work extends this systematic assessing framework for MLLM-as-a-Judge to 15 \textit{Any-to-Any} MMU and MMG tasks, with carefully selected samples for open-ended queries, providing in-depth analysis of potential challenges when applying MLLM-as-a-Judge across broader modalities and more general use cases.
